Guaranteed clustering and biclustering via semidefinite programming

Identifying clusters of similar objects in data plays a significant role in a wide range of applications. As a model problem for clustering, we consider the densest k-disjoint-clique problem, whose goal is to identify the collection of k disjoint cliques of a given weighted complete graph maximizing the sum of the densities of the complete subgraphs induced by these cliques. In this paper, we establish conditions ensuring exact recovery of the densest k cliques of a given graph from the optimal solution of a particular semidefinite program. In particular, the semidefinite relaxation is exact for input graphs corresponding to data consisting of k large, distinct clusters and a smaller number of outliers. This approach also yields a semidefinite relaxation for the biclustering problem with similar recovery guarantees. Given a set of objects and a set of features exhibited by these objects, biclustering seeks to simultaneously group the objects and features according to their expression levels. This problem may be posed as partitioning the nodes of a weighted bipartite complete graph such that the sum of the densities of the resulting bipartite complete subgraphs is maximized. As in our analysis of the densest k-disjoint-clique problem, we show that the correct partition of the objects and features can be recovered from the optimal solution of a semidefinite program in the case that the given data consists of several disjoint sets of objects exhibiting similar features. Empirical evidence from numerical experiments supporting these theoretical guarantees is also provided.

==> Bernstein-proof.tex <==
Denote by $n_i$ the summation $\sum_{j \in I_2} X_{ij}$ for each $i \in I_1$.
We define $\Psi$ to be the event that at least one $n_i$ differs significantly from its mean;
that is, we define $\Psi$ to be the event that there exists $i \in I_1$ such that $n_i >t r_2$
where $t:= 1 + \bar x$.
We let $\tilde \Psi$ denote the complement of $\Psi$, and let $\tilde \psi(n_i)$ be the indicator of this complement.
That is, $\tilde \psi(n_i) = 1$ if $n_i \le t r_2$ and is equal to $0$ otherwise.
We let $B$ be a positive scalar to be determined later.
Note that
\begin{align}
	P\left( \sum_{i\in I_1}  \right. & \left. \frac{ \left| n_i - \bar x r_2 \right|^{\delta}}{r_2} 
		\ge B \frac{r_1}{r_2^{1-\delta/2}} \right) \notag \\
		&\le P \left(\sum_{i\in I_1} \frac{ \left| n_i - \bar x r_2 \right|^{\delta}}{r_2} 
		\ge B \frac{r_1}{r_2^{1-\delta/2}}  \wedge \tilde \Psi \right) + P(\Psi) \label{B: two terms}.
\end{align}
We analyze the two terms separately. To obtain an upper bound on the first term we use a technique of Bernstein (see \cite{Hoeffding}).
Let $\phi$ be the indicator function of the nonnegative reals.
Then
\begin{align*}
	P \left(\sum_{i\in I_1} \right. & \left. \frac{ \left| n_i - \bar x r_2 \right|^{\delta}}{r_2} 
		\ge B \frac{r_1}{r_2^{1-\delta/2}}  \wedge \tilde \Psi \right) \\
	&=P \left(\sum_{i\in I_1} \frac{ \left| n_i - \bar x r_2 \right|^{\delta}}{r_2} 
		- B \frac{r_1}{r_2^{1-\delta/2}} \ge 0 \wedge \tilde \psi(n_i) \; \forall i \in I_1 \right) \\
	&=P \left(\sum_{i\in I_1} \frac{ \left| n_i - \bar x r_2 \right|^{\delta}}{r_2^{\delta/2}} 
		- B r_1 \ge 0 \wedge \tilde \psi(n_i) \; \forall i \in I_1 \right) \\
	&= E \left( \phi \left( \sum_{i\in I_1} \frac{ |n_i - \bar x r_2|^{\delta}}{r_2^{\delta/2}} - Br_1 \right)
		\cdot\prod_{i\in I_1} \tilde \psi(n_i) \right).
\end{align*}
Let $h$ be a positive scalar satisfying $h \le 1/4$. For any $h > 0$ and all $x \in \R$,
$\phi(x) \le \exp(hx)$. By the independence of the $n_i$'s, we have
\begin{align*}
	P \left(\sum_{i\in I_1}  \right. & \left. \frac{ \left| n_i - \bar x r_2 \right|^{\delta}}{r_2} 
		\ge B \frac{r_1}{r_2^{1-\delta/2}}  \wedge \tilde \Psi \right) \\
	&= E \left( \phi \left( \sum_{i\in I_1} \frac{ |n_i - \bar x r_2|^{\delta}}{r_2^{\delta/2}} - Br_1 \right)
		\prod_{i\in I_1} \tilde \psi(n_i) \right) \\
	&\le E \left( \exp\left(h\left( \sum_{i\in I_1} \frac{ |n_i - \bar x r_2|^{\delta}}{r_2^{\delta/2}} - Br_1 \right) \right)
		\cdot\prod_{i\in I_1} \tilde \psi(n_i) \right) \\
	&= \prod_{i\in I_1} E \left(\exp \left( h \left( \frac{|n_i - \bar x r_2|^{\delta}}{r_2^{\delta/2}} - B \right) \right) \tilde \psi(n_i) \right) \\
	&= \prod_{i\in I_1} f_i,
\end{align*}
where
\begin{align} \label{B: f defn}
	f_i &:= E \left(\exp \left( h \left( \frac{|n_i - \bar x r_2|^{\delta}}{r_2^{\delta/2}} - B \right) \right) \tilde \psi(n_i) \right) \\
	&= \int_{0}^{trs} \exp \left( h \left( \frac{|x - \bar x r_2|^{\delta}}{r_2^{\delta/2}} - B \right) \right)g(x)  dx \label{B: f integral}
\end{align}
where $g$ is the probability density function of $n_i$
for all $i\in I_1$.

We analyze each $f_i$ individually. Fix $i \in I_1$.
For each integer, $k = 0, 1,\dots, \floor{t r_2}$, and $x$ such that 
$$
	k \sqrt{r_2} \le |x - \bar x r_2| \le (k+1) \sqrt{r_2},
$$
we overestimate the integrand in \eqref{B: f integral} as
\begin{equation} \label{B: f overest}
	\exp \left( h \left( \frac{|x - \bar x r_2|^{\delta}}{r_2^{\delta/2}} - B \right) \right) 
		P(|x - \bar x r_2| \ge k \sqrt{r_2})
		\le 2\exp( h (k+1)^\delta - hB) \exp(-2k^2)
\end{equation}
by \eqref{Hoeffding-sqrt}.
It follows that
\begin{equation} \label{B: f  sum}
	f_i \le \sum_{k=0}^{\floor{t\sqrt{r_2}}} 2\exp(h(i+1)^\delta - hB - 2k^2).
\end{equation}		
Overestimating the finite sum in \eqref{B: f sum} as an infinite sum and observing that the choice of
$h \le 1/4$ ensures that $h(k+1)^\delta - 2k^2 \le - k^2$ yields
\begin{align}
	f_i & \le 2 \exp(h (1-B)) + 2 \exp(-hB) \sum_{k=1}^\infty \exp(-k^2). \label{B: f inf bound}
\end{align}
Note that $\sum_{k=1}^\infty \exp(-k^2)$ is dominated by a geometric series.
Therefore, for fixed $h \le 1/4$, it is possible to choose $B$, depending only on $h$, so that each
term in \eqref{B: f inf bound} is at most $1/3$ and, hence $f_i \le 2/3$ for all $i \in I_1$. 
It follows immediately that
\begin{equation} \label{B: term 1 bound}
	P \left( \sum_{i \in I_1} \frac{|n_i - \bar x r_2|^{\delta}}{r_2} \ge B \frac{r_1}{r_2^{1-\delta/2}} \wedge \tilde \Psi \right)	
		\le (2/3)^{r_1}.
\end{equation}

We next obtain a bound on the second term in \eqref{B: two terms}.
For any $i \in I_1$, the probability that $|n_i - \bar x r_2| > r_2$ is at most $2\exp(-2 r_2)$ by \eqref{Hoeffding-1}.
Applying the union bound shows that the probability that any $i\in I_1$ satisfies $|n_i - \bar x r_2| > r_2$ is at most
\begin{equation} \label{B: prob psi}
	P(\Psi) \le 2 r_1 \exp(-2 r_2).
\end{equation}
Substituting \eqref{B: term 1  bound} and \eqref{B: prob psi} in \eqref{B: two terms} completes the proof.




		
	


==> b-nonneg-proof.tex <==
% Statement of assumptions.
Let $(U_1,V_1)$, \dots, $(U_k,V_k)$ denote the vertex sets of  a $k$-disjoint-biclique subgraph of the 
bipartite complete graph $K_{M,N} = ((U,V),E)$ with vertex sets $U$ and $V$ of size $M$ and $N$ respectively.
Let $W \in \R^{M\times N}$ be a random nonnegative matrix sampled from the planted bicluster model
according to distributions $\Omega_1, \Omega_2$ with means $\alpha, \beta$.
Let $U_{k+1} = U \setminus (\cup_{i=1}^k U_i)$, $V_{k+1} = V \setminus (\cup_{i=1}^k V_i)$,
$m_i$, $n_i$, $\tau_i$, $C_i$, $r_i$, $\hat m,$ and $\hat n$, be
defined as in Section~\ref{sec: b opt conds} for all $i=1,\dots, k+1$.
Suppose that $\alpha, \beta, \tau_1,\dots, \tau_{k+1}$ satisfy \eqref{eq: a twice b} and \eqref{eq: abd assumption}.
Let $\mu_1, \mu_2, \lambda, \phi, \eta$ be chosen according to
\eqref{eq: mu1 choice}, \eqref{eq: mu2 choice}, \eqref{eq: lambda choice}, \eqref{eq: phi choice}, and \eqref{eq: eta choice}.
In this section, we establish that the entries of $\lambda, \phi,$ and $\eta$ are nonnegative with extremely high probability.

%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
% A lower bound on entries of lambda, phi.
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
We first establish that the multipliers $\lambda$ and $\phi$ are nonnegative with high probability.
The following lemma provides the necessary lower bound on the entries of $\lambda$ and $\phi$.


\begin{lemma}	\label{lem: lower bound on lambda, phi}
	There exist scalars $c_1, c_2 > 0$ depending only on $\alpha, \beta$, $\tau_1,$ \dots, $\tau_k$ such that
	\begin{equation}	\label{eq: lambda, phi bound}
		\lambda_i \ge (c_1 - c_2 \hat n^{-1/4}), \;\;\; \phi_j \ge (c_1 - c_2 \hat n^{-1/4} )
	\end{equation}
	for all $i \in U \setminus U_{k+1},$ $j \in V\setminus V_{k+1}$ with \pteto{\hat n}.
\end{lemma}

\begin{proof}
	Fix $q \in \{1,\dots, k\}$ and $i \in U_q$.
	Recall that
	$$
		\lambda_i = \frac{1}{V_q} \left( \sum_{j \in U_q} \tau_q W_{ij} - \frac{1}{2} \left( \frac{\e^T W_{U_q, V_q} \e}{\tau_q n_q} + \mu_1 \right) \right).
	$$
	% Hoeffding part
	Applying Hoeffding's inequality  \eqref{Hoeffding-1} with $S = \sum_{j\in V_q} W_{ij}$ and $t = n_q^{3/4}$ shows that
	\begin{equation}	\label{eq: lambda hoeffding}
		\left|\sum_{j \in V_q} W_{ij} - \alpha n_q \right| \le n_q^{3/4}
	\end{equation}
	with probability at least $1 - 2 \exp(-2 \hat n^{1/2})$ for all $i \in U_q$.
	% Bernstein part.
	Moreover, applying \eqref{Hoeffding-1} with $S = \e^TW_{U_q, V_q} \e$ and $t = m_q \sqrt{n_q}$ yields
	\begin{equation}	\label{eq: lambda bernstein}
		\e^T W_{U_q, V_q} \e \le \alpha m_q n_q + m_q \sqrt{n_q}
	\end{equation}
	with probability at least $1 - 2 \exp(-2 \hat m)$.	
	Combining \eqref{eq: lambda hoeffding} and \eqref{eq: lambda bernstein} shows that there exist scalars $c_1, c_2>0$ depending only on $\alpha, \beta$, and $\{\tau_1,\dots, \tau_k\}$
	such that
	$$
		\lambda_i  \ge \frac{1}{m_q} \left( \frac{1}{2} (\alpha \tau_q n_q - \mu_1) - 2\tau_q n_q^{3/4} \right) \ge c_1 - c_2 \hat n^{-1/4}
	$$
	with probability at least $ 1- 2 \exp(-2 \hat m) - 2 \exp(-2 \hat n^{1/2})$.
	A similar argument shows that $c_1$ and $c_2$ may be chosen so that
	$$
		\phi_j \ge c_1 - c_2 \hat n^{-1/4}
	$$
	with probability at least $ 1- 2 \exp(-2 \hat m) - 2 \exp(-2 \hat n^{1/2})$ for each $j \in V_q$.
	Applying the union bound over all $i \in U$, $j\in V$ completes the proof.
	\qed
\end{proof}

%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
% Lower bound on eta.
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
We now derive lower bounds on the entries of $\eta$.
Recall that $\eta(C_q, C_s) = \Pi^{q,s} - \y^{q,s} \w_s^T - \w_q ( \z^{q,s}  )^T$ for all $q \neq s$,
where the entries of the matrix $\Pi^{q,s}$ are bounded below by a positive scalar with \pteto{\hat n}. All remaining entries of $\eta$ are  $0$.
Therefore, to prove that $\eta$ is nonnegative with high probability, 
it suffices to  shows that the entries of $\y^{q,s}$ and $\z^{q,s}$ tend to zero with high probability as $\hat n$ approaches $\infty$.
The following lemma provides the necessary upper bound on $\|\y^{q,s}\|_\infty$ and $\|\z^{q,s}\|_\infty$.

% Upper bound on inf norm of  y, z.
\begin{lemma}	\label{lem: bicluster y,z inf bounds}
	There exists scalar $c > 0$ such that
	\begin{equation} \label{eq: B yz inf bound}
		\|\y^{q,s} \|_\infty + \| \z^{q,s} \|_{\infty} \le c \hat n^{-1/4}
	\end{equation}
	for all $q,s \in \{1,\dots, k\}$ such that $q\neq s$ with \pteto{\hat n}.
\end{lemma}

\begin{proof}
	% Plan of attack.
	Fix $q,s \in \{1,\dots, k\}$ such that $q\neq s$.
	The proof for the case when $q$ or $s$ is equal to $k+1$ follows by a similar argument.
	Without loss of generality, we may assume that $n_q \le n_s$.
	We first obtain an upper bound on $\|\y\|_\infty = \|\y^{q,s}\|_\infty$.
	Recall that
	$$
		\y =  \frac{1}{2m_s} \rbra{ I - \frac{\w_q \w_q^T}{2(m_q + m_s) } } \b_{C_q}.
	$$	
	By the triangle inequality, we have
	\begin{equation*}
		\|\y\|_\infty \le  \frac{1}{2 m_s} \rbra{ \|\b_{C_q} \|_\infty+ \frac{ \|\w_q\|_\infty  }{2(m_q + m_s)} |\b_{C_q}^T \w_q|  }
			=  \frac{1}{2 m_s} \rbra{ \|\b_{C_q} \|_\infty+ \frac{ \max\{1, \tau_q\} }{ 2(m_q + m_s) } |\b_{C_q}^T \w_q| }.		
	\end{equation*}
	Therefore, it suffices to show that $\|\b_{C_q}\|_\infty = O(\sqrt{n_s})$ and that $| \b_{C_q}^T \w_q |$ is bounded above by a scalar
	multiple of $n_s \sqrt{n_q}$ with probability tending exponentially to $1$ as $\hat n$ approaches $\infty$.
	
	% Bound on |b_{C_q}^T e|.
	We begin by deriving the necessary upper bound on $|\b_{C_q}^T \w_q |$.
	Recall that 
	\begin{align*}
		\b_{C_q} 
			&= \mat{ {c} m_s ( \lambda_{U_q} - E[\lambda_{U_q}] )+ \big( ( \lambda_{U_s} - E[\lambda_{U_s} ] )^T\e \big)\e  - \tau_s( W_{U_q, V_s}\e - \beta n_s \e) \\
				- (W_{U_s, V_q}^T \e	 - \beta m_s \e )   + \tau_s \Big( n_s (\phi_{V_q} - E[\phi_{V_q}]) +  \big((\phi_{V_s} - E [\phi_{V_s}])^T \e\big) \e \Big)}			
	\end{align*}
	Taking the inner product of $\b_{C_q}$ with $\w_q$ yields
	\begin{align}
		\b_{C_q}^T \w_q 	= \frac{\tau_q}{2 m_q} ( m_s + \tau_q \tau_s n_s) & (\e^T W_{U_q,V_q} \e - \alpha m_q n_q )
				+ \frac{\tau_s}{2m_s}(m_q + \tau_q\tau_s n_q) ( \e^T W_{U_s, V_s} \e - \alpha m_s n_s )  \notag\\
				-& \tau_s (\e^T W_{U_q, V_s} \e - \beta m_q n_s ) -  \tau_q (\e^T W_{U_s, V_q} \e - \beta m_s n_q ).  \label{eq: bCq*e expansion}
	\end{align}
	% Bernstein bounds.
	Recall that $| \e^T W_{U_q, V_q} \e - \alpha m_q n_q |  \le  m_q \sqrt{n_q}$ and $| \e^T W_{U_s, V_s} \e - \alpha m_s n_s | \le  m_s \sqrt{n_s}$
	with probability at least $ 1 - 2 p_1$ by \eqref{eq: lambda bernstein},
	where $p_1:= 2 \exp(-2 \hat m)$.
	Applying \eqref{Hoeffding-1} with $S = \e^T W_{U_q, V_s} \e$ and $t = m_q \sqrt{n_s}$
	shows that
	\begin{equation}	\label{eq: upper right block sum}
		| \e^T W_{U_q, V_s} \e - \beta m_q n_s | \le m_q \sqrt{n_s}
	\end{equation}
	with probability at least $1 - p_1$.
	Similarly,  applying \eqref{Hoeffding-1} with $S = \e^T W_{U_s, V_q} \e$ and $t = n_q \sqrt{m_s}$ yields
	\begin{equation}	\label{eq: lower left block sum}
		| \e^T W_{U_s, V_q} \e - \beta m_s n_q  | \le n_q \sqrt{m_s}
	\end{equation}
	with probability at least $1 - 2 \exp(-2 \hat n) =:1 - p_2$.
	Applying the triangle inequality and the union bound to \eqref{eq: bCq*e expansion} shows that
	\begin{equation}  \label{eq: b_Cq 1 norm bound}
		|\b_{C_q}^T \w_q | \le  c_1  n_s\sqrt{n_q}
	\end{equation}
	for some scalar $c_1 > 0$  with probability at least $1 - 3p_1 - p_2$.
	Similarly, there exists scalar $c_2 > 0$ such that $|\b_{C_s}^T \w_s | \le  c_2 n_s\sqrt{n_q}$
	with probability at least $1 - 3 p_1 - p_2$.
	
	%  Bound on infnorm(b).
	We next derive an upper bound on $\|\b_{C_q} \|_\infty$.
	By the triangle inequality,
	\begin{equation}	\label{eq: b inf norm triangle}
		\|\b_{U_q} \|_\infty \le m_s \|\lambda_{U_q} - E[\lambda_{U_q}] \|_{\infty} 
					+ |(\lambda_{U_s} - E[\lambda_{U_s}])^T \e|
					- \tau_s \| W_{U_q, V_s} \e - \beta n_s \e \|_\infty.
	\end{equation}
	Recall that
	$$
		\lambda_i - E[\lambda_i] = \frac{1}{m_q} \rbra{ \tau_q \rbra{ \sum_{j\in V_q} W_{ij} - \alpha n_q } - \frac{1}{2\tau_q n_q} \rbra{ \e^T W_{U_q, V_q} \e - \alpha m_q n_q } }
	$$
	for all $i \in U_q$. 
	Applying \eqref{eq: lambda hoeffding}, \eqref{eq: lambda bernstein},  and the union bound over all $i \in U_q$ shows that
	\begin{equation} \label{eq: lambda inf norm}
	\|\lambda_{U_q} - E[\lambda_{U_q}] \|_{\infty}  \le  \tilde c_1 {n_q^{-1/4}}
	\end{equation}
	for some scalar $\tilde c_1 > 0$,
	with probability at least $1 - p_1 - 2 m_q \exp(-2 \hat n^{1/2})$.	
	Similarly,
	\begin{equation} \label{eq: lambda sum bound}
		|(\lambda_{U_s} - E[\lambda_{U_s}])^T \e | \le \frac{\tau_s }{2m_s} \left|{ \e^T W_{U_s, V_s} \e - \alpha m_s n_s} \right| \le \frac{\tau_s}{2} \sqrt{n_s}
	\end{equation}
	with probability at least $1- p_1$ by \eqref{eq: lambda bernstein}.
	Finally, \eqref{eq: lambda hoeffding} implies that	
	\begin{equation} \label{eq: b inf bound W pt}
		\left| \sum_{j\in V_s} W_{ij} - \beta n_s \right| \le n_s^{3/4}
	\end{equation}
	for all $i \in U_q$
	with probability at least $1- 2 m_q \exp(-2 n^{1/2})$.
	Substituting \eqref{eq: lambda inf norm}, \eqref{eq: lambda sum bound}, and \eqref{eq: b inf bound W pt} into \eqref{eq: b inf norm triangle}
	shows that there exists scalar $\tilde c_2 > 0$ such that
	$$
		\|\b_{U_q} \|_\infty \le \tilde c_2 n_s n_q^{-1/4}
	$$
	with \pteto{\hat n}.
	Following a similar argument, one can show that $\| \b_{V_q} \|_\infty$ and $\|\b_{C_s}\|_\infty$ are bounded above by scalar multiples of $n_sn_q^{-1/4}$ and $n_q^{3/4}$, respectively,
	with \pteto{\hat n}.	
	% Put everything together.	
	It follows that there exists scalar $c > 0$ such that	
	\begin{equation} 	\label{eq: z inf norm bound}
		\|\y \|_\infty  \le (c/2) n_q^{-1/4} 
	\end{equation}
	with  \pteto{\hat n}.
	By a similar argument, $\|\z\|_\infty \le (c/2) n_q^{-1/4}$ with probability tending exponentially to $1$ as $\hat n$ approaches $\infty$.
	Applying the union bound one last time completes the proof.
	\qed
	\bigskip
\end{proof}

	
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
% Uniqueness condition holds.
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
Lemmas~\ref{lem: lower bound on lambda, phi}  and \ref{lem: bicluster y,z inf bounds} imply that $\lambda, \phi,$ and $\eta$
are nonnegative with probability tending exponentially to $1$ as $\hat n$ tends to $\infty$.
Therefore, if the planted bicliques $(U_1, V_1),\dots, (U_k, V_k)$ satisfy  \eqref{eq: S1 bound cond} 
 then the corresponding feasible solution $Z^*$ is optimal for \eqref{eq: WKDB relaxation} with \pteto{\hat n} by Theorem~\ref{thm: WKDB sufficient}.
The following theorem states that the uniqueness condition given by \eqref{eq: bicluster uniqueness cond} is also satisfied with high probability by 
matrices $W$ sampled from the planted bicluster model.

\begin{lemma}	\label{thm: unique cond holds}
	For all $q,s \in \{1,\dots, k\}$ such that $q \neq s$,
	$$
		n_s \e^T W_{U_q V_q} \e - n_q \e^T W_{U_q, V_s} \e \ge m_q n_q n_s ( \alpha - \beta - (n_q^{-1/2} + n_s^{-1/2}) ) 
	$$
	with \pteto{\hat n}.
%	There exists scalar $c>0$ such that
%	$$
%		n_s \e^T W_{U_q V_q} \e - n_q \e^T W_{U_q, V_s} \e \ge m_q n_q n_s ( \alpha - \beta - c (n_q^{-1/2} + n_s^{-1/2}) ) 
%	$$
%	for all $q,s \in \{1,\dots, k\}$ such that $q \neq s$ with \pteto{\hat n}.
\end{lemma}

\begin{proof}
	Fix $q \neq s$. Recall that 
	$$
		\e^T W_{U_q, V_q} \e \ge \alpha m_q n_q -  m_q n_q^{1/2}
	$$
	with probability at least $1-p_1$ by \eqref{eq: lambda bernstein}.
	Moreover,
	$$
		\e^T W_{U_q, V_s} \e \le  \beta m_q n_s + m_q n_s^{1/2}
	$$
	with probability at least $1-p_1$ by \eqref{eq: upper right block sum}.
	It follows immediately that
	$$
		n_s \e^T W_{U_q V_q} \e - n_q \e^T W_{U_q, V_s} \e \ge m_q n_q n_s ( \alpha - \beta -  (n_q^{-1/2} + n_s^{-1/2}) ) 
	$$
	with probability at least $1 - 2 p_1$. Applying the union bound over all $q \neq s$ completes the proof.
	\qed
\end{proof}
	
	
	
	
	
	
	
	
	
	
	
	
	
	
	
	
	

==> background.tex <==
%%%
% Geman
We first recall a theorem of Geman \cite{Geman:1980} providing a bound on the spectral norm of
a random matrix with \iid  entries of mean $0$. 

\begin{theorem}
    \label{geman tail bound}
    Let $A$ be a $\lceil yn \rceil \times n$ random matrix with \iid entries sampled
    from a  distribution with mean $\mu$ and variance $\sigma^2$ such that 
    $A_{ij} \in [0,1]$ for all $i \in \{1,\dots, \ceil{yn}\}$, $j \in \{1, \dots, n\}$
    for fixed $y \in \R_+$.
    Then, with probability at least $1 - c_1 \exp(-c_2 n^{c_3})$
    where $c_1 > 0$, $c_2>0$, and $c_3 > 0$  depend on $\sigma$ and $y$,
    $$
        \|A - \mu \e\e^T \| \le c_4 \sigma \sqrt{n}
    $$
    for some $c_4>0$ depending on $y$.
\end{theorem}

Note that this theorem is not stated in this form in \cite{Geman:1980},
but can be deduced from the equations on
pp.~255--256 by taking $k=n^q$ for a $q$ satisfying $(2\alpha+4)q<1$.

%%%%%
% Furedi and Komlos.				
A similar theorem due to F\"uredi and Koml\'os \cite{Furedi-Komlos:1981} 
is available for symmetric matrices.

\begin{theorem}
    \label{Furedi-Komlos}
        Let $A \in \Sigma^n$ be a random symmetric matrix with \iid entries sampled from a distribution 
        with mean $\mu$ and variance $\sigma^2$ such that $A_{ij} \in [0,1]$ for all $i,j \in \{1,\dots, n\}$.
        Then
	$$
            	\| A - \mu \e\e^T \| \le 3 \sigma\sqrt{n}
	$$
	with probability at least $1 - \exp(-c  n^{1/6})$ where $c$ depends only on $\sigma$.
\end{theorem}

As in the case of Geman's paper \cite{Geman:1980}, this theorem is not stated exactly this
way in \cite{Furedi-Komlos:1981}, 
but can be deduced by taking $k = \sigma^{1/3} n^{1/6}$ and $v = \sigma \sqrt{n}$
in the inequality
$$
	P(\max |\lambda| > 2 \sigma\sqrt{n} + v) < \sqrt{n} \exp(-kv/(2 \sigma \sqrt{n} + v))
$$
on pp. 237 of  \cite{Furedi-Komlos:1981}.

%%%%%%%
% Hoeffding.
We conclude with a theorem of 

%The final theorem of this section provides a bound on the $\ell_1$ and $\ell_2$ norms of random vectors whose entries are equal to the sum of
%bounded \iid random variables.
%
%
%\begin{theorem}
%	\label{thm: Bernstein}
%	Let $I_1, I_2$ be index sets of size $r_1, r_2$ respectively.
%	Let $\{X_{ij}: i \in I_1, j \in I_2\}$ be a collection of \iid random variables with mean $\bar X$
%	such that $0 \le X_{ij} \le 1$ for all $i \in I_1$, $j \in I_2$.
%	Then there exists scalar $B$ such that
%	\begin{equation}
%		\label{eqn: Bernstein}
%		\sum_{i\in I_1} {\left|\sum_{j\in I_2} X_{ij} - r_2 \bar X \right|^\delta} \le
%		 	B {r_1 r_2^{\delta/2}}
%	\end{equation}
%	with probability at least
%	\begin{equation} \label{eqn: Bernstein prob}
%		1 - (2/3)^{r_1} - 2 r_1 \exp(-2 r_2) 
%	\end{equation}
%	for $\delta = 1,2$.
%\end{theorem}
%
%The proof of Theorem~\ref{thm: Bernstein} is a modification of the proof of Lemma~4.1 in \cite{AV2}
%and is included in Appendix~\ref{sec: thm 2.4 proof}.
